Theoretical and phenomenological consequences of active and sterile neutrino within Beyond Standard Model framework

This thesis address theoretical and phenomenological aspects of active and sterile mixing pattern within minimal extended seesaw frameworks. It consists of six chapters, where chapters one and six are dedicated to introduction and conclusion chapters, respectively. In chapter two, we study active-sterile phenomenology with a single generation of sterile neutrino ($m_S\sim \mathcal{O}$(eV)) along with the three active neutrinos. Three independent cases for sterile mass matrices are studied in both normal and inverted hierarchy mass ordering. Chapter three is an extension of the previous chapter. The neutrino mass generation and baryogenesis {\it via} thermal leptogenesis are studied in the fermionic sector. On the other hand, an extended multi Higgs doublet model is studied in the scalar sector. Among the three Higgs doublet, one of them does not acquire any vacuum expectation value (VEV); hence, it behaves as an inert Higgs. The lightest component of this behaves as a viable dark matter candidate. Within MES, sterile mass can be stressed up to the $keV$ scale. In the fourth chapter, we studied various phenomenologies considering sterile neutrino mass in the $keV$ range. This $keV$ scaled sterile neutrino also plays the role of dark matter candidate in our study. The fifth chapter is dedicated to the texture-zero neutrino dark matter model. We study active-sterile mixing, baryogenesis $via$ resonant leptogenesis and $0\nu\beta\beta$ in the fermion sector. While, in the scalar sector, the complex scalar flavon that gives rise to sterile mass takes part in dark matter study. The imaginary component of that scalar flavon is behaving as a viable dark matter candidate.

==> Chapters/Abstract.tex <==
\begin{document}
	adcd
\end{document}
A d d

==> Chapters/Chap8.tex <==

\chapter*{} % Main chapter title
\vspace{-2.1cm}

%{\it ``After five years' work I allowed myself to speculate on the subject, and drew up some short notes; these I enlarged in 1844 into a sketch of the conclusions, which then seemed to me probable: from that period to the present day I have steadily pursued the same object. I hope that I may be excused for entering on these personal details, as I give them to show that I have not been hasty in coming to a decision."---{ \Large Charles Darwin}}

%\label{Chapter7} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

%\lhead{Chapter 7. \emph{Conclusion and future plan}} % Change X to a consecutive number; this is for the header on each page - perhaps a shortened title

%----------------------------------------------------------------------------------------
%	SECTION 1
%----------------------------------------------------------------------------------------
\section{Conferences, School,  Workshop attended}

\vspace{-0.8cm}
\rule{\textwidth}{0.4pt}
\begin{itemize}
	\item{\bf School:} Attended {\bf DST-SERB School on Theoretical High Energy Physics}, held at University of Hyderabad, Aug 20- Sept 16, 2018.
	\item{\bf School:} Attended {\bf Summer School on Particle Physics}, held at ICTP, Italy from 10-21 June, 2019.
	\item {\bf Conference:}
	POSTER PRESENTED AT {\bf XIV National Conference on HEP } HELD AT
	GAUHATI UNIVERSITY, INDIA FROM MARCH 21-23, 2018.
	\item {\bf Conference:}
	POSTER PRESENTED AT {\bf XXIII DAE-BRNS HIGH ENERGY SYMPOSIUM 2018} HELD AT
	IIT MADRAS, INDIA FROM DECEMBER 10-14, 2018.
	\item {\bf Workshop:} Attended {\bf XVI WORKSHOP ON HIGH ENERGY PHYSICS PHENOMENOLOGY} HELD AT IIT GUWAHATI, 1-10 DECEMBER,2019.
	\item {\bf Int. Conference:}
	CONTRIBUTORY TALK  AT {\bf EICP-2} HELD AT
	VISHWA BHARATI, KOLKATA, INDIA FROM JANUARY 10-14, 2020.
	\item {\bf Conference:}
	POSTER PRESENTATION \& PARALLEL SESSION TALK AT {\bf XXIV DAE-BRNS HIGH ENERGY SYMPOSIUM 2018} HELD AT
	NISER, BHUBNESHWAR, INDIA FROM DECEMBER 14-17, 2020.
\end{itemize}
\clearpage
\section{\Large List of publications}
%		\skip
\rule{\textwidth}{0.4pt}
\begin{enumerate}
	\item
	{\bf Das P.}, Mukherjee A., Das M. K.; {\it Active and sterile neutrino phenomenology with $A_4$ based minimal extended seesaw}, {\bf Nuclear Physics B, Volume 941, April 2019, Pages 755-779}; arxiv:1805.092132
	\item{\bf Das P.}, Das M. K.,{\it  Phenomenology of $keV$ sterile neutrino within minimal extended seesaw}. arXiv: 1908.08417. {\bf IJMPA; Vol. 35, No. 22, 2050125 (2020)}
	\item {\bf Das P.}, Das M. K., Khan N. {\it Influence of multi-Higgs doublet in scalar and fermionic sector within minimal extended seesaw  framework}. arXiv: 1911.07243. {\bf JHEP; 2020, Article number: 18 (2020) }
	\item {\bf Das P.}, Das M. K., Khan N.; {\it A new feasible dark matter region in the singlet scalar scotogenic model.} {\bf  Nuclear Physics B;
		Volume 964, March 2021, 115307} ({\it 		arXiv:2001.04070})
	\item  Sarma L., {\bf Das P.}, Das M. K.; {\it Scalar dark matter and leptogenesis in the minimal scotogenic model.} {\bf Nuclear Physics B;
		Volume 963, February 2021, 115300
	} arXiv:2004.13762
	\item {\bf Das P.}, Das M. K., Khan N.; {\it Five-zero texture in neutrino-dark matter model within the framework of minimal extended seesaw.} {\bf arXiv:2010.13084} ({\it Under communication})
\end{enumerate}

==> Chapters/Chapter2.tex <==
% Chapter Template

\chapter{Discrete flavour symmetry and neutrino mass models} % Main chapter title

\label{Chapter2.1} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

\lhead{Chapter 2.1 \emph{Discrete flavour symmetry and neutrino mass models}} % Change X to a consecutive number; this is for the header on each page - perhaps a shortened title

%----------------------------------------------------------------------------------------
%	SECTION 1
%----------------------------------------------------------------------------------------


%%
%
%
%
%
%









\section{Conclusion}
This chapter has discussed four models that we have constructed using $A_4$ and $Z_n (n\ge2)$ discrete symmetries. Models are focused on active-sterile mixing pattern with different scales of sterile mass and study phenomenological consequences in both experimental and observable sectors. Except the {\bf neutrino mass model I}, various kinds of dark matter candidates are also addressed in all other models. In {\bf neutrino mass model II} and {\bf neutrino mass model IV}, both real and complex scalar dark matters are discussed respectively, on the other hand in {\bf neutrino mass model III}, $keV$ sterile neutrino as a fermionic dark matter candidate is addressed. In the following chapters, we will be discussing numerical results for individual models. 
